Lung Cancer Lesion Detection in Histopathology Images Using Graph-Based Sparse PCA Network

Early detection of lung cancer is critical for improvement of patient survival. To address the clinical need for efficacious treatments, genetically engineered mouse models (GEMM) have become integral in identifying and evaluating the molecular underpinnings of this complex disease that may be exploited as therapeutic targets. Assessment of GEMM tumor burden on histopathological sections performed by manual inspection is both time consuming and prone to subjective bias. Therefore, an interplay of needs and challenges exists for computer-aided diagnostic tools, for accurate and efficient analysis of these histopathology images. In this paper, we propose a simple machine learning approach called the graph-based sparse principal component analysis (GS-PCA) network, for automated detection of cancerous lesions on histological lung slides stained by hematoxylin and eosin (H&E). Our method comprises four steps: 1) cascaded graph-based sparse PCA, 2) PCA binary hashing, 3) block-wise histograms, and 4) support vector machine (SVM) classification. In our proposed architecture, graph-based sparse PCA is employed to learn the filter banks of the multiple stages of a convolutional network. This is followed by PCA hashing and block histograms for indexing and pooling. The meaningful features extracted from this GS-PCA are then fed to an SVM classifier. We evaluate the performance of the proposed algorithm on H&E slides obtained from an inducible K-rasG12D lung cancer mouse model using precision/recall rates, F-score, Tanimoto coefficient, and area under the curve (AUC) of the receiver operator characteristic (ROC) and show that our algorithm is efficient and provides improved detection accuracy compared to existing algorithms.

==> README <==

December 27, 2012


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

V1.8 is a significant update over the 1.7a release. For a full list of
changes, please read the file changelog.txt. The most notable changes
include:


 1) New transmag class option to support the IEEE Transactions on Magnetics
    format. Thanks to Wei Yingkang, Sangmin Suh and Benjamin Gaussens
    for suggestions and beta testing.

 2) The \IEEEcompsoctitleabstractindextext and 
    \IEEEdisplaynotcompsoctitleabstractindextext
    commands have been deprecated in favor of their
    \IEEEtitleabstractindextext and \IEEEdisplaynontitleabstractindextext
    (observe that the "not" has changed to "non") equivalents. This change
    generalizes and decouples them from compsoc mode because the new
    transmag mode also uses them now.

 3) Added new *-forms of \IEEEyesnumber*, \IEEEnonumber*, \IEEEyessubnumber*,
    and \IEEEnosubnumber* (the non-star form of the latter is also new) which
    persist across IEEEeqnarray lines until countermanded. To provide for
    continued subequations across instances of IEEEeqnarrays as well as for
    subequations that follow a main equation (e.g., 14, 14a, 14b ...)
    \IEEEyessubnumber no longer automatically increments the equation number
    on it's first invocation of a subequation group. Invoke both
    \IEEEyesnumber\IEEEyessubnumber together to start a new
    equation/subequation group.
 
 4) Hyperref links now work with IEEEeqnarray equations.
    Thanks to Stefan M. Moser for reporting this problem.

 5) Revised spacing at top of top figures and tables to better
    align with the top main text lines as IEEE does in its journals. 
    Thanks to Dirk Beyer for reporting this issue and beta testing.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> README_BST <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> different_refs.tex <==
%--------------------------------------------------------------------------------------------------------------------------------------------------%
%%%Hanley82%%
%@article{hanley1982meaning,
%  title={The meaning and use of the area under a receiver operating characteristic ({ROC}) curve.},
%  author={Hanley, James A and McNeil, Barbara J},
%  journal={Radiology},
%  volume={143},
%  number={1},
%  pages={29--36},
%  year={1982}
%}

%%%Floyd62%%
%@article{floyd1962algorithm,
%  title={Algorithm 97: shortest path},
%  author={Floyd, Robert W},
%  journal={Communications of the ACM},
%  volume={5},
%  number={6},
%  pages={345},
%  year={1962},
%  publisher={ACM}
%}

%%%French82%%
%@book{french1982sequencing,
%  title={Sequencing and scheduling: an introduction to the mathematics of the job-shop},
%  author={French, Simon},
%  volume={683},
%  year={1982},
%  publisher={Ellis Horwood Chichester}
%}

%%%Otto03%%
%@article{otto2003mutations,
%  title={Mutations in INVS encoding inversin cause nephronophthisis type 2, linking renal cystic disease to the function of primary cilia and left-right axis determination},
%  author={E. A. Otto and B. Schermer and T. Obara and J. F. O\'Toole and K. S. Hiller and A. M. Mueller and R. G. Ruf and J. Hoefele and F. Beekmann and D. Landau and J. W. Foreman and J. A. Goodship and T. Strachan and A. Kispert and M. T. Wolf and M. F. Gagnadoux and H. Nivet and C. Antignac and G. Walz and I. A. Drummond and T. Benzing and F. Hildebrandt},
%  journal={Nature Genetics},
%  volume={34},
%  number={4},
%  pages={413--420},
%  year={2003},
%  publisher={Nature Publishing Group}
%}

%%%Singla06%%
%@article{singla2006primary,
%  title={The primary cilium as the cell's antenna: signaling at a sensory organelle},
%  author={Singla, Veena and Reiter, Jeremy F},
%  journal={Science},
%  volume={313},
%  number={5787},
%  pages={629--633},
%  year={2006},
%  publisher={American Association for the Advancement of Science}
%}

%%%Verghese09%%
%@article{verghese2009renal,
%  title={Renal primary cilia lengthen after acute tubular necrosis},
%  author={Verghese, Elizabeth and Ricardo, Sharon D and Weidenfeld, Raphael and Zhuang, Junli and Hill, Prudence A and Langham, Robyn G and Deane, James A},
%  journal={Journal of the American Society of Nephrology},
%  volume={20},
%  number={10},
%  pages={2147--2153},
%  year={2009},
%  publisher={Am Soc Nephrol}
%}

%%%Miyoshi09%%
%@article{miyoshi2009lithium,
%  title={Lithium treatment elongates primary cilia in the mouse brain and in cultured cells},
%  author={Miyoshi, Ko and Kasahara, Kyosuke and Miyazaki, Ikuko and Asanuma, Masato},
%  journal={Biochemical and biophysical research communications},
%  volume={388},
%  number={4},
%  pages={757--762},
%  year={2009},
%  publisher={Elsevier}
%}

%%%Miyoshi11%%
% @article{miyoshi2011factors,
%  title={Factors that influence primary cilium length},
%  author={Miyoshi, Ko and Kasahara, Kyosuke and Miyazaki, Ikuko and Asanuma, Masato},
%  journal={Acta Med Okayama},
%  volume={65},
%  pages={279--285},
%  year={2011}
%}

%%%Telea02%%
% @inproceedings{telea2002augmented,
%  title={An augmented fast marching method for computing skeletons and centerlines},
%  author={Telea, Alexandru and Van Wijk, Jarke J},
%  booktitle={Proceedings of the Symposium on Data Visualisation 2002},
%  pages={251--ff},
%  year={2002},
%  organization={Eurographics Association}
%}

%%%Vapnik98%%
%@book{vapnik1998statistical,
%  title={Statistical learning theory},
%  author={Vapnik, Vladimir Naumovich and Vapnik, Vlamimir},
%  volume={1},
%  year={1998},
%  publisher={Wiley New York}
%}

%%%Macqueen67%%
%@inproceedings{macqueen1967some,
%  title={Some methods for classification and analysis of multivariate observations},
%  author={MacQueen, James and others},
%  booktitle={Proceedings of the fifth Berkeley symposium on mathematical statistics and probability},
%  volume={1},
%  number={14},
%  pages={281--297},
%  year={1967},
%  organization={Oakland, CA, USA.}
%}

%%%Lloyd82%%
%@article{lloyd1982least,
%  title={Least squares quantization in PCM},
%  author={Lloyd, Stuart P},
%  journal={Information Theory, IEEE Transactions on},
%  volume={28},
%  number={2},
%  pages={129--137},
%  year={1982},
%  publisher={IEEE}
%}

%%%Singla06%%
%@article{singla2006primary,
%  title={The primary cilium as the cell's antenna: signaling at a sensory organelle},
%  author={Singla, Veena and Reiter, Jeremy F},
%  journal={science},
%  volume={313},
%  number={5787},
%  pages={629--633},
%  year={2006},
%  publisher={American Association for the Advancement of Science}
%}

% %%Yoder07%%
% @article{yoder2007role,
%  title={Role of primary cilia in the pathogenesis of polycystic kidney disease},
%  author={Yoder, Bradley K},
%  journal={Journal of the American Society of Nephrology},
%  volume={18},
%  number={5},
%  pages={1381--1388},
%  year={2007},
%  publisher={Am Soc Nephrol}
%}

%%%Choi97%%
%@article{choi1997mathematical,
%  title={Mathematical theory of medial axis transform},
%  author={Choi, Hyeong In and Choi, Sung Woo and Moon, Hwan Pyo},
%  journal={Pacific Journal of Mathematics},
%  volume={181},
%  number={1},
%  pages={57--88},
%  year={1997}
%}
 
%%%Dijkstra59%%
%@article{dijkstra1959note,
%  title={A note on two problems in connexion with graphs},
%  author={Dijkstra, Edsger W},
%  journal={Numerische Mathematik},
%  volume={1},
%  number={1},
%  pages={269--271},
%  year={1959},
%  publisher={Springer}
%}

%%%Fukunaga75%%
%@article{fukunaga1975estimation,
%  title={The estimation of the gradient of a density function, with applications in pattern recognition},
%  author={Fukunaga, Keinosuke and Hostetler, Larry D},
%  journal={Information Theory, IEEE Transactions on},
%  volume={21},
%  number={1},
%  pages={32--40},
%  year={1975},
%  publisher={IEEE}
%}

%%%Deledalle09%%
%@article{deledalle2009iterative,
%  title={Iterative weighted maximum likelihood denoising with probabilistic patch-based weights},
%  author={Deledalle, Charles-Alban and Denis, Lo{\"\i}c and Tupin, Florence},
%  journal=J_IEEE_IP,
%  volume={18},
%  number={12},
%  pages={2661--2672},
%  year={2009},
%  publisher={IEEE}
%}

%%%Russell95%%
%@article{russell1995artificial,
%  title={Artificial intelligence: a modern approach},
%  author={Russell, Stuart and Norvig, Peter},
%  year={1995}
%}

%%%Jianbo15%%
%@MastersThesis{Jianbo:Thesis:2015,
%    author     =     {Jianbo Shao},
%    title     =     {{Analysis and modeling of primary cilia in microscopy images}},
%    school     =     {The university of arizona},
%    year     =     {2015},
% }

%%%Veland09%%
%@article{veland2009primary,
%  title={Primary cilia and signaling pathways in mammalian development, health and disease},
%  author={Veland, Iben R and Awan, Aashir and Pedersen, Lotte B and Yoder, Bradley K and Christensen, S{\o}ren T},
%  journal={Nephron Physiology},
%  volume={111},
%  number={3},
%  pages={p39--p53},
%  year={2009},
%  publisher={Karger Publishers}
%}
 
%%%Gerdes09%%
% @article{gerdes2009vertebrate,
%  title={The vertebrate primary cilium in development, homeostasis, and disease},
%  author={Gerdes, Jantje M and Davis, Erica E and Katsanis, Nicholas},
%  journal={Cell},
%  volume={137},
%  number={1},
%  pages={32--45},
%  year={2009},
%  publisher={Elsevier}
%}

%%%Filegauf07%%
%@article{fliegauf2007cilia,
%  title={When cilia go bad: cilia defects and ciliopathies},
%  author={Fliegauf, Manfred and Benzing, Thomas and Omran, Heymut},
%  journal={Nat. Rev. Mol. Cell Biol.},
%  volume={8},
%  number={11},
%  pages={880--893},
%  year={2007},
%  publisher={Nature Publishing Group}
%}

%%%Strack98%%
%@book{Starck:1998:IPD:289385,
% author = {Starck, J.-L. and Murtagh, F. and Bijaoui, A.},
% title = {Image Processing and Data Analysis: The Multiscale Approach},
% year = {1998},
% isbn = {0-521-59914-8},
% publisher = {Cambridge University Press},
% address = {New York, NY, USA},
%} 

%%%Zeng06%%
%@article{zeng2006detecting,
%  title={Detecting and measuring fine roots in minirhizotron images using matched filtering and local entropy thresholding},
%  author={Zeng, Guang and Birchfield, Stanley T and Wells, Christina E},
%  journal={Machine Vision and Applications},
%  volume={17},
%  number={4},
%  pages={265--278},
%  year={2006},
%  publisher={Springer}
%}

%%%Kohavi95%%
%@inproceedings{kohavi1995study,
%  title={A study of cross-validation and bootstrap for accuracy estimation and model selection},
%  author={Kohavi, Ron and others},
%  booktitle={Ijcai},
%  volume={14},
%  number={2},
%  pages={1137--1145},
%  year={1995}
%}

%%%Van07%%
%@article{van2007subvoxel,
%  title={Subvoxel precise skeletons of volumetric data based on fast marching methods},
%  author={Van Uitert, Robert and Bitter, Ingmar},
%  journal={Medical Physics},
%  volume={34},
%  number={2},
%  pages={627--638},
%  year={2007},
%  publisher={American Association of Physicists in Medicine}
%}

%%%Schneider12%%
%@article{schneider2012nih,
%  title={NIH Image to ImageJ: 25 years of image analysis},
%  author={Schneider, Caroline A and Rasband, Wayne S and Eliceiri, Kevin W},
%  journal={Nature Methods},
%  volume={9},
%  number={7},
%  pages={671--675},
%  year={2012},
%  publisher={Nature Publishing Group}
%}

%%%Sethian96%%
%@article{sethian1996fast,
%  title={A fast marching level set method for monotonically advancing fronts},
%  author={Sethian, James A},
%  journal={Proceedings of the National Academy of Sciences},
%  volume={93},
%  number={4},
%  pages={1591--1595},
%  year={1996},
%  publisher={National Acad Sciences}
%}




